Measurement of the charged-particle multiplicity inside jets from $\sqrt{s}=8$ TeV $pp$ collisions with the ATLAS detector

The number of charged particles inside jets is a widely used discriminant for identifying the quark or gluon nature of the initiating parton and is sensitive to both the perturbative and non-perturbative components of fragmentation. This paper presents a measurement of the average number of charged particles with $p_\text{T}>500$ MeV inside high-momentum jets in dijet events using 20.3 fb$^{-1}$ of data recorded with the ATLAS detector in $pp$ collisions at $\sqrt{s}=8$ TeV collisions at the LHC. The jets considered have transverse momenta from 50 GeV up to and beyond 1.5 TeV. The reconstructed charged-particle track multiplicity distribution is unfolded to remove distortions from detector effects and the resulting charged-particle multiplicity is compared to several models. Furthermore, quark and gluon jet fractions are used to extract the average charged-particle multiplicity for quark and gluon jets separately.

==> figures/systs_Mean_all_Central_3_PDF_CT10_PAPER.tex <==
\begin{table}[h]
\begin{tabular}{lclcllllllll}
 {\bf Average $n_\text{charged}$} & \multicolumn{10}{c}{Jet $p_\text{T}$ Range {[}100 GeV{]}} \\
\begin{tabular}[c]{@{}c@{}}Systematic\\[-3mm] Uncertainty [\%]\end{tabular} & {[}0.5,1{]}          & {[}1,2{]}             & {[}2,3{]}            & {[}3,4{]}             & {[}4,5{]}             & {[}5,6{]}             & {[}6,8{]}             & {[}8,10{]}            & {[}10,12{]}           & {[}12,15{]}       & {[}15,18{]}     \\ \hline
Response Matrix\\\hspace{5mm}Total Jet Energy Scale & \multicolumn{1}{c}{${}^{+  1.6}_{-  1.8}$}
& \multicolumn{1}{c}{${}^{+  0.8}_{-  0.7}$}
& \multicolumn{1}{c}{${}^{+  0.4}_{-  0.5}$}
& \multicolumn{1}{c}{${}^{+  0.5}_{-  0.5}$}
& \multicolumn{1}{c}{${}^{+  0.3}_{-  0.3}$}
& \multicolumn{1}{c}{${}^{+  0.2}_{-  0.2}$}
& \multicolumn{1}{c}{${}^{+  0.2}_{-  0.2}$}
& \multicolumn{1}{c}{${}^{+  0.1}_{-  0.1}$}
& \multicolumn{1}{c}{${}^{+  0.1}_{-  0.1}$}
& \multicolumn{1}{c}{${}^{+  0.1}_{-  0.1}$}
& \multicolumn{1}{c}{${}^{+  0.2}_{-  0.4}$}
\\
\hspace{5mm}Jet Energy Resolution & \multicolumn{1}{c}{${}^{+  0.4}_{-  0.4}$}
& \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.1}_{-  0.1}$}
& \multicolumn{1}{c}{${}^{+  0.1}_{-  0.1}$}
& \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
\\
\hspace{5mm}Charged Energy Loss & \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  1.2}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  1.1}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  1.1}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  1.1}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  1.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  3.7}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  3.3}_{-  0.0}$}
\\
\hspace{5mm}Other Tracking & \multicolumn{1}{c}{${}^{+  0.8}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.6}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.6}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.6}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.6}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.6}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.6}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.6}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.6}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.7}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.7}_{-  0.0}$}
\\
Correction Factors & \multicolumn{1}{c}{${}^{+  0.6}_{-  0.6}$}
& \multicolumn{1}{c}{${}^{+  0.3}_{-  0.3}$}
& \multicolumn{1}{c}{${}^{+  0.2}_{-  0.2}$}
& \multicolumn{1}{c}{${}^{+  0.1}_{-  0.1}$}
& \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.1}_{-  0.1}$}
& \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
\\
Unfolding Procedure& \multicolumn{1}{c}{${}^{+  5.8}_{-  5.8}$}
& \multicolumn{1}{c}{${}^{+  3.6}_{-  3.6}$}
& \multicolumn{1}{c}{${}^{+  0.7}_{-  0.7}$}
& \multicolumn{1}{c}{${}^{+  0.8}_{-  0.8}$}
& \multicolumn{1}{c}{${}^{+  0.5}_{-  0.5}$}
& \multicolumn{1}{c}{${}^{+  0.4}_{-  0.4}$}
& \multicolumn{1}{c}{${}^{+  0.4}_{-  0.4}$}
& \multicolumn{1}{c}{${}^{+  0.3}_{-  0.3}$}
& \multicolumn{1}{c}{${}^{+  0.3}_{-  0.3}$}
& \multicolumn{1}{c}{${}^{+  0.2}_{-  0.2}$}
& \multicolumn{1}{c}{${}^{+  0.2}_{-  0.2}$}
\\
\hline
Total Systematic & \multicolumn{1}{c}{${}^{+  6.1}_{-  6.1}$}
& \multicolumn{1}{c}{${}^{+  3.7}_{-  3.7}$}
& \multicolumn{1}{c}{${}^{+  1.0}_{-  0.9}$}
& \multicolumn{1}{c}{${}^{+  1.2}_{-  1.0}$}
& \multicolumn{1}{c}{${}^{+  1.5}_{-  0.6}$}
& \multicolumn{1}{c}{${}^{+  1.4}_{-  0.5}$}
& \multicolumn{1}{c}{${}^{+  1.3}_{-  0.4}$}
& \multicolumn{1}{c}{${}^{+  1.3}_{-  0.3}$}
& \multicolumn{1}{c}{${}^{+  1.2}_{-  0.3}$}
& \multicolumn{1}{c}{${}^{+  3.7}_{-  0.2}$}
& \multicolumn{1}{c}{${}^{+  3.4}_{-  0.4}$}
\\
Data Statistics & \multicolumn{1}{c}{  0.5}
& \multicolumn{1}{c}{  0.2}
& \multicolumn{1}{c}{  0.1}
& \multicolumn{1}{c}{  0.1}
& \multicolumn{1}{c}{  0.0}
& \multicolumn{1}{c}{  0.1}
& \multicolumn{1}{c}{  0.1}
& \multicolumn{1}{c}{  0.2}
& \multicolumn{1}{c}{  0.6}
& \multicolumn{1}{c}{  1.2}
& \multicolumn{1}{c}{  3.3}
\\
Total Uncertainty & \multicolumn{1}{c}{${}^{+  6.1}_{-  6.1}$}
& \multicolumn{1}{c}{${}^{+  3.7}_{-  3.7}$}
& \multicolumn{1}{c}{${}^{+  1.0}_{-  0.9}$}
& \multicolumn{1}{c}{${}^{+  1.2}_{-  1.0}$}
& \multicolumn{1}{c}{${}^{+  1.5}_{-  0.6}$}
& \multicolumn{1}{c}{${}^{+  1.4}_{-  0.5}$}
& \multicolumn{1}{c}{${}^{+  1.3}_{-  0.5}$}
& \multicolumn{1}{c}{${}^{+  1.3}_{-  0.4}$}
& \multicolumn{1}{c}{${}^{+  1.4}_{-  0.7}$}
& \multicolumn{1}{c}{${}^{+  3.9}_{-  1.2}$}
& \multicolumn{1}{c}{${}^{+  4.7}_{-  3.3}$}
\\
\hline\hline
Measured Value& \multicolumn{1}{c}{ 7.91}
& \multicolumn{1}{c}{10.23}
& \multicolumn{1}{c}{12.90}
& \multicolumn{1}{c}{14.56}
& \multicolumn{1}{c}{15.70}
& \multicolumn{1}{c}{16.53}
& \multicolumn{1}{c}{17.28}
& \multicolumn{1}{c}{18.17}
& \multicolumn{1}{c}{18.88}
& \multicolumn{1}{c}{19.05}
& \multicolumn{1}{c}{20.32}
\\
\end{tabular}
\caption{A summary of all the systematic uncertainties and their impact on the $n_\text{track}$ mean for $p_\text{T}^\text{track}>0.5$ GeV and the more central jet.  Uncertainties are given in percent. A value of 0.0 is quoted if the uncertainty is below 0.05\%.}
\label{tab:systs_Mean_all_Central_3}
\end{table} 


==> figures/systs_Mean_all_Central_5_PDF_CT10_PAPER.tex <==
\begin{table}[h]
\begin{tabular}{lclcllllllll}
 {\bf Average $n_\text{charged}$} & \multicolumn{10}{c}{Jet $p_\text{T}$ Range {[}100 GeV{]}} \\
\begin{tabular}[c]{@{}c@{}}Systematic\\[-3mm] Uncertainty [\%]\end{tabular} & {[}0.5,1{]}          & {[}1,2{]}             & {[}2,3{]}            & {[}3,4{]}             & {[}4,5{]}             & {[}5,6{]}             & {[}6,8{]}             & {[}8,10{]}            & {[}10,12{]}           & {[}12,15{]}       & {[}15,18{]}     \\ \hline
Response Matrix\\\hspace{5mm}Total Jet Energy Scale & \multicolumn{1}{c}{${}^{+  2.1}_{-  2.5}$}
& \multicolumn{1}{c}{${}^{+  1.0}_{-  1.0}$}
& \multicolumn{1}{c}{${}^{+  0.5}_{-  0.7}$}
& \multicolumn{1}{c}{${}^{+  0.6}_{-  0.6}$}
& \multicolumn{1}{c}{${}^{+  0.4}_{-  0.4}$}
& \multicolumn{1}{c}{${}^{+  0.3}_{-  0.3}$}
& \multicolumn{1}{c}{${}^{+  0.3}_{-  0.3}$}
& \multicolumn{1}{c}{${}^{+  0.2}_{-  0.2}$}
& \multicolumn{1}{c}{${}^{+  0.2}_{-  0.1}$}
& \multicolumn{1}{c}{${}^{+  0.1}_{-  0.1}$}
& \multicolumn{1}{c}{${}^{+  0.3}_{-  0.4}$}
\\
\hspace{5mm}Jet Energy Resolution & \multicolumn{1}{c}{${}^{+  0.7}_{-  0.7}$}
& \multicolumn{1}{c}{${}^{+  0.1}_{-  0.1}$}
& \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.1}_{-  0.1}$}
& \multicolumn{1}{c}{${}^{+  0.1}_{-  0.1}$}
& \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.1}_{-  0.1}$}
& \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
\\
\hspace{5mm}Charged Energy Loss & \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  1.2}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  1.1}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  1.1}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  1.1}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  1.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  3.7}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  3.3}_{-  0.0}$}
\\
\hspace{5mm}Other Tracking & \multicolumn{1}{c}{${}^{+  0.7}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.6}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.6}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.6}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.6}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.6}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.6}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.6}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.6}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.7}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.8}_{-  0.0}$}
\\
Correction Factors & \multicolumn{1}{c}{${}^{+  0.3}_{-  0.3}$}
& \multicolumn{1}{c}{${}^{+  0.2}_{-  0.2}$}
& \multicolumn{1}{c}{${}^{+  0.2}_{-  0.2}$}
& \multicolumn{1}{c}{${}^{+  0.1}_{-  0.1}$}
& \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.1}_{-  0.1}$}
& \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
\\
Unfolding Procedure& \multicolumn{1}{c}{${}^{+  5.3}_{-  5.3}$}
& \multicolumn{1}{c}{${}^{+  3.6}_{-  3.6}$}
& \multicolumn{1}{c}{${}^{+  0.7}_{-  0.7}$}
& \multicolumn{1}{c}{${}^{+  0.7}_{-  0.7}$}
& \multicolumn{1}{c}{${}^{+  0.5}_{-  0.5}$}
& \multicolumn{1}{c}{${}^{+  0.4}_{-  0.4}$}
& \multicolumn{1}{c}{${}^{+  0.4}_{-  0.4}$}
& \multicolumn{1}{c}{${}^{+  0.3}_{-  0.3}$}
& \multicolumn{1}{c}{${}^{+  0.2}_{-  0.2}$}
& \multicolumn{1}{c}{${}^{+  0.3}_{-  0.3}$}
& \multicolumn{1}{c}{${}^{+  0.1}_{-  0.1}$}
\\
\hline
Total Systematic & \multicolumn{1}{c}{${}^{+  5.8}_{-  5.9}$}
& \multicolumn{1}{c}{${}^{+  3.8}_{-  3.8}$}
& \multicolumn{1}{c}{${}^{+  1.1}_{-  1.0}$}
& \multicolumn{1}{c}{${}^{+  1.1}_{-  0.9}$}
& \multicolumn{1}{c}{${}^{+  1.5}_{-  0.7}$}
& \multicolumn{1}{c}{${}^{+  1.3}_{-  0.5}$}
& \multicolumn{1}{c}{${}^{+  1.3}_{-  0.5}$}
& \multicolumn{1}{c}{${}^{+  1.3}_{-  0.4}$}
& \multicolumn{1}{c}{${}^{+  1.2}_{-  0.3}$}
& \multicolumn{1}{c}{${}^{+  3.8}_{-  0.3}$}
& \multicolumn{1}{c}{${}^{+  3.4}_{-  0.4}$}
\\
Data Statistics & \multicolumn{1}{c}{  0.5}
& \multicolumn{1}{c}{  0.2}
& \multicolumn{1}{c}{  0.1}
& \multicolumn{1}{c}{  0.1}
& \multicolumn{1}{c}{  0.0}
& \multicolumn{1}{c}{  0.1}
& \multicolumn{1}{c}{  0.1}
& \multicolumn{1}{c}{  0.2}
& \multicolumn{1}{c}{  0.7}
& \multicolumn{1}{c}{  1.3}
& \multicolumn{1}{c}{  3.4}
\\
Total Uncertainty & \multicolumn{1}{c}{${}^{+  5.8}_{-  6.0}$}
& \multicolumn{1}{c}{${}^{+  3.9}_{-  3.8}$}
& \multicolumn{1}{c}{${}^{+  1.1}_{-  1.0}$}
& \multicolumn{1}{c}{${}^{+  1.1}_{-  0.9}$}
& \multicolumn{1}{c}{${}^{+  1.5}_{-  0.7}$}
& \multicolumn{1}{c}{${}^{+  1.3}_{-  0.5}$}
& \multicolumn{1}{c}{${}^{+  1.3}_{-  0.5}$}
& \multicolumn{1}{c}{${}^{+  1.3}_{-  0.4}$}
& \multicolumn{1}{c}{${}^{+  1.4}_{-  0.7}$}
& \multicolumn{1}{c}{${}^{+  4.0}_{-  1.3}$}
& \multicolumn{1}{c}{${}^{+  4.8}_{-  3.4}$}
\\
\hline\hline
Measured Value& \multicolumn{1}{c}{ 4.96}
& \multicolumn{1}{c}{ 7.06}
& \multicolumn{1}{c}{ 9.64}
& \multicolumn{1}{c}{11.27}
& \multicolumn{1}{c}{12.43}
& \multicolumn{1}{c}{13.30}
& \multicolumn{1}{c}{14.12}
& \multicolumn{1}{c}{15.12}
& \multicolumn{1}{c}{15.93}
& \multicolumn{1}{c}{16.18}
& \multicolumn{1}{c}{17.45}
\\
\end{tabular}
\caption{A summary of all the systematic uncertainties and their impact on the $n_\text{track}$ mean for $p_\text{T}^\text{track}>2$ GeV and the more central jet.  Uncertainties are given in percent. A value of 0.0 is quoted if the uncertainty is below 0.05\%.}
\label{tab:systs_Mean_all_Central_5}
\end{table} 


==> figures/systs_Mean_all_Central_7_PDF_CT10_PAPER.tex <==
\begin{table}[h]
\begin{tabular}{lclcllllllll}
 {\bf Average $n_\text{charged}$} & \multicolumn{10}{c}{Jet $p_\text{T}$ Range {[}100 GeV{]}} \\
\begin{tabular}[c]{@{}c@{}}Systematic\\[-3mm] Uncertainty [\%]\end{tabular} & {[}0.5,1{]}          & {[}1,2{]}             & {[}2,3{]}            & {[}3,4{]}             & {[}4,5{]}             & {[}5,6{]}             & {[}6,8{]}             & {[}8,10{]}            & {[}10,12{]}           & {[}12,15{]}       & {[}15,18{]}     \\ \hline
Response Matrix\\\hspace{5mm}Total Jet Energy Scale & \multicolumn{1}{c}{${}^{+  3.6}_{-  4.1}$}
& \multicolumn{1}{c}{${}^{+  1.6}_{-  1.5}$}
& \multicolumn{1}{c}{${}^{+  0.7}_{-  0.8}$}
& \multicolumn{1}{c}{${}^{+  0.7}_{-  0.7}$}
& \multicolumn{1}{c}{${}^{+  0.5}_{-  0.5}$}
& \multicolumn{1}{c}{${}^{+  0.4}_{-  0.4}$}
& \multicolumn{1}{c}{${}^{+  0.3}_{-  0.3}$}
& \multicolumn{1}{c}{${}^{+  0.2}_{-  0.3}$}
& \multicolumn{1}{c}{${}^{+  0.2}_{-  0.2}$}
& \multicolumn{1}{c}{${}^{+  0.1}_{-  0.1}$}
& \multicolumn{1}{c}{${}^{+  0.2}_{-  0.3}$}
\\
\hspace{5mm}Jet Energy Resolution & \multicolumn{1}{c}{${}^{+  1.5}_{-  1.5}$}
& \multicolumn{1}{c}{${}^{+  0.3}_{-  0.3}$}
& \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.1}_{-  0.1}$}
& \multicolumn{1}{c}{${}^{+  0.1}_{-  0.1}$}
& \multicolumn{1}{c}{${}^{+  0.1}_{-  0.1}$}
& \multicolumn{1}{c}{${}^{+  0.1}_{-  0.1}$}
& \multicolumn{1}{c}{${}^{+  0.1}_{-  0.1}$}
& \multicolumn{1}{c}{${}^{+  0.1}_{-  0.1}$}
& \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
\\
\hspace{5mm}Charged Energy Loss & \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  1.2}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  1.1}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  1.1}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  1.1}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  1.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  3.7}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  3.4}_{-  0.0}$}
\\
\hspace{5mm}Other Tracking & \multicolumn{1}{c}{${}^{+  0.7}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.6}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.6}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.6}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.6}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.6}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.6}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.6}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.7}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.7}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.9}_{-  0.0}$}
\\
Correction Factors & \multicolumn{1}{c}{${}^{+  1.0}_{-  1.0}$}
& \multicolumn{1}{c}{${}^{+  0.2}_{-  0.2}$}
& \multicolumn{1}{c}{${}^{+  0.2}_{-  0.2}$}
& \multicolumn{1}{c}{${}^{+  0.1}_{-  0.1}$}
& \multicolumn{1}{c}{${}^{+  0.1}_{-  0.1}$}
& \multicolumn{1}{c}{${}^{+  0.1}_{-  0.1}$}
& \multicolumn{1}{c}{${}^{+  0.1}_{-  0.1}$}
& \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.1}_{-  0.1}$}
& \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
\\
Unfolding Procedure& \multicolumn{1}{c}{${}^{+  5.1}_{-  5.1}$}
& \multicolumn{1}{c}{${}^{+  3.1}_{-  3.1}$}
& \multicolumn{1}{c}{${}^{+  0.6}_{-  0.6}$}
& \multicolumn{1}{c}{${}^{+  0.6}_{-  0.6}$}
& \multicolumn{1}{c}{${}^{+  0.4}_{-  0.4}$}
& \multicolumn{1}{c}{${}^{+  0.4}_{-  0.4}$}
& \multicolumn{1}{c}{${}^{+  0.3}_{-  0.3}$}
& \multicolumn{1}{c}{${}^{+  0.3}_{-  0.3}$}
& \multicolumn{1}{c}{${}^{+  0.2}_{-  0.2}$}
& \multicolumn{1}{c}{${}^{+  0.2}_{-  0.2}$}
& \multicolumn{1}{c}{${}^{+  0.2}_{-  0.2}$}
\\
\hline
Total Systematic & \multicolumn{1}{c}{${}^{+  6.6}_{-  6.8}$}
& \multicolumn{1}{c}{${}^{+  3.6}_{-  3.5}$}
& \multicolumn{1}{c}{${}^{+  1.1}_{-  1.0}$}
& \multicolumn{1}{c}{${}^{+  1.1}_{-  0.9}$}
& \multicolumn{1}{c}{${}^{+  1.5}_{-  0.7}$}
& \multicolumn{1}{c}{${}^{+  1.3}_{-  0.6}$}
& \multicolumn{1}{c}{${}^{+  1.3}_{-  0.5}$}
& \multicolumn{1}{c}{${}^{+  1.3}_{-  0.4}$}
& \multicolumn{1}{c}{${}^{+  1.3}_{-  0.3}$}
& \multicolumn{1}{c}{${}^{+  3.7}_{-  0.2}$}
& \multicolumn{1}{c}{${}^{+  3.5}_{-  0.3}$}
\\
Data Statistics & \multicolumn{1}{c}{  0.6}
& \multicolumn{1}{c}{  0.2}
& \multicolumn{1}{c}{  0.1}
& \multicolumn{1}{c}{  0.0}
& \multicolumn{1}{c}{  0.0}
& \multicolumn{1}{c}{  0.1}
& \multicolumn{1}{c}{  0.1}
& \multicolumn{1}{c}{  0.2}
& \multicolumn{1}{c}{  0.6}
& \multicolumn{1}{c}{  1.2}
& \multicolumn{1}{c}{  3.5}
\\
Total Uncertainty & \multicolumn{1}{c}{${}^{+  6.6}_{-  6.8}$}
& \multicolumn{1}{c}{${}^{+  3.6}_{-  3.5}$}
& \multicolumn{1}{c}{${}^{+  1.1}_{-  1.0}$}
& \multicolumn{1}{c}{${}^{+  1.1}_{-  0.9}$}
& \multicolumn{1}{c}{${}^{+  1.5}_{-  0.7}$}
& \multicolumn{1}{c}{${}^{+  1.3}_{-  0.6}$}
& \multicolumn{1}{c}{${}^{+  1.3}_{-  0.5}$}
& \multicolumn{1}{c}{${}^{+  1.3}_{-  0.5}$}
& \multicolumn{1}{c}{${}^{+  1.4}_{-  0.7}$}
& \multicolumn{1}{c}{${}^{+  3.9}_{-  1.2}$}
& \multicolumn{1}{c}{${}^{+  5.0}_{-  3.5}$}
\\
\hline\hline
Measured Value& \multicolumn{1}{c}{ 2.41}
& \multicolumn{1}{c}{ 4.07}
& \multicolumn{1}{c}{ 6.27}
& \multicolumn{1}{c}{ 7.76}
& \multicolumn{1}{c}{ 8.86}
& \multicolumn{1}{c}{ 9.73}
& \multicolumn{1}{c}{10.56}
& \multicolumn{1}{c}{11.62}
& \multicolumn{1}{c}{12.45}
& \multicolumn{1}{c}{12.84}
& \multicolumn{1}{c}{13.93}
\\
\end{tabular}
\caption{A summary of all the systematic uncertainties and their impact on the $n_\text{track}$ mean for $p_\text{T}^\text{track}>5$ GeV and the more central jet.  Uncertainties are given in percent. A value of 0.0 is quoted if the uncertainty is below 0.05\%.}
\label{tab:systs_Mean_all_Central_7}
\end{table} 


==> figures/systs_Mean_all_Forward_5_PDF_CT10_PAPER.tex <==
\begin{table}[h]
\begin{tabular}{lclcllllllll}
 {\bf Average $n_\text{charged}$} & \multicolumn{10}{c}{Jet $p_\text{T}$ Range {[}100 GeV{]}} \\
\begin{tabular}[c]{@{}c@{}}Systematic\\[-3mm] Uncertainty [\%]\end{tabular} & {[}0.5,1{]}          & {[}1,2{]}             & {[}2,3{]}            & {[}3,4{]}             & {[}4,5{]}             & {[}5,6{]}             & {[}6,8{]}             & {[}8,10{]}            & {[}10,12{]}           & {[}12,15{]}       & {[}15,18{]}     \\ \hline
Response Matrix\\\hspace{5mm}Total Jet Energy Scale & \multicolumn{1}{c}{${}^{+  2.4}_{-  2.6}$}
& \multicolumn{1}{c}{${}^{+  1.2}_{-  1.3}$}
& \multicolumn{1}{c}{${}^{+  0.7}_{-  0.9}$}
& \multicolumn{1}{c}{${}^{+  0.9}_{-  0.8}$}
& \multicolumn{1}{c}{${}^{+  0.7}_{-  0.8}$}
& \multicolumn{1}{c}{${}^{+  0.7}_{-  0.7}$}
& \multicolumn{1}{c}{${}^{+  0.7}_{-  0.7}$}
& \multicolumn{1}{c}{${}^{+  0.6}_{-  0.5}$}
& \multicolumn{1}{c}{${}^{+  0.4}_{-  0.5}$}
& \multicolumn{1}{c}{${}^{+  0.4}_{-  0.4}$}
& \multicolumn{1}{c}{${}^{+  0.8}_{-  0.7}$}
\\
\hspace{5mm}Jet Energy Resolution & \multicolumn{1}{c}{${}^{+  1.0}_{-  1.0}$}
& \multicolumn{1}{c}{${}^{+  0.1}_{-  0.1}$}
& \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.2}_{-  0.2}$}
& \multicolumn{1}{c}{${}^{+  0.1}_{-  0.1}$}
& \multicolumn{1}{c}{${}^{+  0.1}_{-  0.1}$}
& \multicolumn{1}{c}{${}^{+  0.1}_{-  0.1}$}
& \multicolumn{1}{c}{${}^{+  0.2}_{-  0.2}$}
& \multicolumn{1}{c}{${}^{+  0.1}_{-  0.1}$}
& \multicolumn{1}{c}{${}^{+  0.1}_{-  0.1}$}
& \multicolumn{1}{c}{${}^{+  0.2}_{-  0.2}$}
\\
\hspace{5mm}Charged Energy Loss & \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  1.2}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  1.1}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  1.1}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  1.1}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  1.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  3.6}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  3.3}_{-  0.0}$}
\\
\hspace{5mm}Other Tracking & \multicolumn{1}{c}{${}^{+  1.1}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.9}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.8}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.8}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.7}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.7}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.7}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.7}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.7}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.8}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.9}_{-  0.0}$}
\\
Correction Factors & \multicolumn{1}{c}{${}^{+  0.1}_{-  0.1}$}
& \multicolumn{1}{c}{${}^{+  0.1}_{-  0.1}$}
& \multicolumn{1}{c}{${}^{+  0.1}_{-  0.1}$}
& \multicolumn{1}{c}{${}^{+  0.1}_{-  0.1}$}
& \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.1}_{-  0.1}$}
& \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.1}_{-  0.1}$}
\\
Unfolding Procedure& \multicolumn{1}{c}{${}^{+  5.8}_{-  5.8}$}
& \multicolumn{1}{c}{${}^{+  3.6}_{-  3.6}$}
& \multicolumn{1}{c}{${}^{+  0.6}_{-  0.6}$}
& \multicolumn{1}{c}{${}^{+  0.8}_{-  0.8}$}
& \multicolumn{1}{c}{${}^{+  0.5}_{-  0.5}$}
& \multicolumn{1}{c}{${}^{+  0.4}_{-  0.4}$}
& \multicolumn{1}{c}{${}^{+  0.4}_{-  0.4}$}
& \multicolumn{1}{c}{${}^{+  0.3}_{-  0.3}$}
& \multicolumn{1}{c}{${}^{+  0.2}_{-  0.2}$}
& \multicolumn{1}{c}{${}^{+  0.1}_{-  0.1}$}
& \multicolumn{1}{c}{${}^{+  0.3}_{-  0.3}$}
\\
\hline
Total Systematic & \multicolumn{1}{c}{${}^{+  6.5}_{-  6.5}$}
& \multicolumn{1}{c}{${}^{+  3.9}_{-  3.8}$}
& \multicolumn{1}{c}{${}^{+  1.3}_{-  1.1}$}
& \multicolumn{1}{c}{${}^{+  1.4}_{-  1.1}$}
& \multicolumn{1}{c}{${}^{+  1.7}_{-  1.0}$}
& \multicolumn{1}{c}{${}^{+  1.6}_{-  0.9}$}
& \multicolumn{1}{c}{${}^{+  1.5}_{-  0.8}$}
& \multicolumn{1}{c}{${}^{+  1.4}_{-  0.6}$}
& \multicolumn{1}{c}{${}^{+  1.3}_{-  0.5}$}
& \multicolumn{1}{c}{${}^{+  3.7}_{-  0.4}$}
& \multicolumn{1}{c}{${}^{+  3.5}_{-  0.8}$}
\\
Data Statistics & \multicolumn{1}{c}{  0.5}
& \multicolumn{1}{c}{  0.2}
& \multicolumn{1}{c}{  0.1}
& \multicolumn{1}{c}{  0.1}
& \multicolumn{1}{c}{  0.0}
& \multicolumn{1}{c}{  0.1}
& \multicolumn{1}{c}{  0.1}
& \multicolumn{1}{c}{  0.3}
& \multicolumn{1}{c}{  0.6}
& \multicolumn{1}{c}{  1.2}
& \multicolumn{1}{c}{  3.7}
\\
Total Uncertainty & \multicolumn{1}{c}{${}^{+  6.5}_{-  6.5}$}
& \multicolumn{1}{c}{${}^{+  3.9}_{-  3.8}$}
& \multicolumn{1}{c}{${}^{+  1.3}_{-  1.1}$}
& \multicolumn{1}{c}{${}^{+  1.4}_{-  1.1}$}
& \multicolumn{1}{c}{${}^{+  1.7}_{-  1.0}$}
& \multicolumn{1}{c}{${}^{+  1.6}_{-  0.9}$}
& \multicolumn{1}{c}{${}^{+  1.5}_{-  0.8}$}
& \multicolumn{1}{c}{${}^{+  1.5}_{-  0.7}$}
& \multicolumn{1}{c}{${}^{+  1.5}_{-  0.8}$}
& \multicolumn{1}{c}{${}^{+  3.9}_{-  1.3}$}
& \multicolumn{1}{c}{${}^{+  5.1}_{-  3.8}$}
\\
\hline\hline
Measured Value& \multicolumn{1}{c}{ 4.93}
& \multicolumn{1}{c}{ 6.88}
& \multicolumn{1}{c}{ 9.16}
& \multicolumn{1}{c}{10.55}
& \multicolumn{1}{c}{11.61}
& \multicolumn{1}{c}{12.46}
& \multicolumn{1}{c}{13.35}
& \multicolumn{1}{c}{14.53}
& \multicolumn{1}{c}{15.40}
& \multicolumn{1}{c}{16.05}
& \multicolumn{1}{c}{17.96}
\\
\end{tabular}
\caption{A summary of all the systematic uncertainties and their impact on the $n_\text{track}$ mean for $p_\text{T}^\text{track}>2$ GeV and the more forward jet.  Uncertainties are given in percent. A value of 0.0 is quoted if the uncertainty is below 0.05\%.}
\label{tab:systs_Mean_all_Forward_5}
\end{table} 


==> figures/systs_Mean_all_Forward_7_PDF_CT10_PAPER.tex <==
\begin{table}[h]
\begin{tabular}{lclcllllllll}
 {\bf Average $n_\text{charged}$} & \multicolumn{10}{c}{Jet $p_\text{T}$ Range {[}100 GeV{]}} \\
\begin{tabular}[c]{@{}c@{}}Systematic\\[-3mm] Uncertainty [\%]\end{tabular} & {[}0.5,1{]}          & {[}1,2{]}             & {[}2,3{]}            & {[}3,4{]}             & {[}4,5{]}             & {[}5,6{]}             & {[}6,8{]}             & {[}8,10{]}            & {[}10,12{]}           & {[}12,15{]}       & {[}15,18{]}     \\ \hline
Response Matrix\\\hspace{5mm}Total Jet Energy Scale & \multicolumn{1}{c}{${}^{+  3.9}_{-  4.2}$}
& \multicolumn{1}{c}{${}^{+  1.8}_{-  1.9}$}
& \multicolumn{1}{c}{${}^{+  0.9}_{-  1.0}$}
& \multicolumn{1}{c}{${}^{+  1.0}_{-  1.0}$}
& \multicolumn{1}{c}{${}^{+  0.9}_{-  0.9}$}
& \multicolumn{1}{c}{${}^{+  0.9}_{-  0.8}$}
& \multicolumn{1}{c}{${}^{+  0.7}_{-  0.8}$}
& \multicolumn{1}{c}{${}^{+  0.7}_{-  0.6}$}
& \multicolumn{1}{c}{${}^{+  0.5}_{-  0.5}$}
& \multicolumn{1}{c}{${}^{+  0.5}_{-  0.5}$}
& \multicolumn{1}{c}{${}^{+  1.0}_{-  0.8}$}
\\
\hspace{5mm}Jet Energy Resolution & \multicolumn{1}{c}{${}^{+  1.8}_{-  1.8}$}
& \multicolumn{1}{c}{${}^{+  0.3}_{-  0.3}$}
& \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.2}_{-  0.2}$}
& \multicolumn{1}{c}{${}^{+  0.1}_{-  0.1}$}
& \multicolumn{1}{c}{${}^{+  0.2}_{-  0.2}$}
& \multicolumn{1}{c}{${}^{+  0.1}_{-  0.1}$}
& \multicolumn{1}{c}{${}^{+  0.2}_{-  0.2}$}
& \multicolumn{1}{c}{${}^{+  0.1}_{-  0.1}$}
& \multicolumn{1}{c}{${}^{+  0.1}_{-  0.1}$}
& \multicolumn{1}{c}{${}^{+  0.3}_{-  0.3}$}
\\
\hspace{5mm}Charged Energy Loss & \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  1.2}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  1.1}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  1.1}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  1.1}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  1.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  3.6}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  3.3}_{-  0.0}$}
\\
\hspace{5mm}Other Tracking & \multicolumn{1}{c}{${}^{+  1.1}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.9}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.8}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.8}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.7}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.7}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.7}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.7}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.8}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.8}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.9}_{-  0.0}$}
\\
Correction Factors & \multicolumn{1}{c}{${}^{+  0.9}_{-  0.9}$}
& \multicolumn{1}{c}{${}^{+  0.2}_{-  0.2}$}
& \multicolumn{1}{c}{${}^{+  0.1}_{-  0.1}$}
& \multicolumn{1}{c}{${}^{+  0.1}_{-  0.1}$}
& \multicolumn{1}{c}{${}^{+  0.1}_{-  0.1}$}
& \multicolumn{1}{c}{${}^{+  0.1}_{-  0.1}$}
& \multicolumn{1}{c}{${}^{+  0.1}_{-  0.1}$}
& \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.1}_{-  0.1}$}
& \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
& \multicolumn{1}{c}{${}^{+  0.0}_{-  0.0}$}
\\
Unfolding Procedure& \multicolumn{1}{c}{${}^{+  5.9}_{-  5.9}$}
& \multicolumn{1}{c}{${}^{+  2.8}_{-  2.8}$}
& \multicolumn{1}{c}{${}^{+  0.4}_{-  0.4}$}
& \multicolumn{1}{c}{${}^{+  0.6}_{-  0.6}$}
& \multicolumn{1}{c}{${}^{+  0.4}_{-  0.4}$}
& \multicolumn{1}{c}{${}^{+  0.4}_{-  0.4}$}
& \multicolumn{1}{c}{${}^{+  0.3}_{-  0.3}$}
& \multicolumn{1}{c}{${}^{+  0.3}_{-  0.3}$}
& \multicolumn{1}{c}{${}^{+  0.1}_{-  0.1}$}
& \multicolumn{1}{c}{${}^{+  0.1}_{-  0.1}$}
& \multicolumn{1}{c}{${}^{+  0.3}_{-  0.3}$}
\\
\hline
Total Systematic & \multicolumn{1}{c}{${}^{+  7.4}_{-  7.5}$}
& \multicolumn{1}{c}{${}^{+  3.4}_{-  3.4}$}
& \multicolumn{1}{c}{${}^{+  1.3}_{-  1.1}$}
& \multicolumn{1}{c}{${}^{+  1.4}_{-  1.2}$}
& \multicolumn{1}{c}{${}^{+  1.7}_{-  1.0}$}
& \multicolumn{1}{c}{${}^{+  1.6}_{-  0.9}$}
& \multicolumn{1}{c}{${}^{+  1.5}_{-  0.9}$}
& \multicolumn{1}{c}{${}^{+  1.5}_{-  0.7}$}
& \multicolumn{1}{c}{${}^{+  1.4}_{-  0.6}$}
& \multicolumn{1}{c}{${}^{+  3.7}_{-  0.5}$}
& \multicolumn{1}{c}{${}^{+  3.6}_{-  0.9}$}
\\
Data Statistics & \multicolumn{1}{c}{  0.7}
& \multicolumn{1}{c}{  0.2}
& \multicolumn{1}{c}{  0.1}
& \multicolumn{1}{c}{  0.1}
& \multicolumn{1}{c}{  0.0}
& \multicolumn{1}{c}{  0.1}
& \multicolumn{1}{c}{  0.1}
& \multicolumn{1}{c}{  0.3}
& \multicolumn{1}{c}{  0.6}
& \multicolumn{1}{c}{  1.3}
& \multicolumn{1}{c}{  3.8}
\\
Total Uncertainty & \multicolumn{1}{c}{${}^{+  7.5}_{-  7.6}$}
& \multicolumn{1}{c}{${}^{+  3.4}_{-  3.4}$}
& \multicolumn{1}{c}{${}^{+  1.3}_{-  1.1}$}
& \multicolumn{1}{c}{${}^{+  1.4}_{-  1.2}$}
& \multicolumn{1}{c}{${}^{+  1.7}_{-  1.0}$}
& \multicolumn{1}{c}{${}^{+  1.6}_{-  0.9}$}
& \multicolumn{1}{c}{${}^{+  1.5}_{-  0.9}$}
& \multicolumn{1}{c}{${}^{+  1.5}_{-  0.7}$}
& \multicolumn{1}{c}{${}^{+  1.5}_{-  0.8}$}
& \multicolumn{1}{c}{${}^{+  4.0}_{-  1.4}$}
& \multicolumn{1}{c}{${}^{+  5.3}_{-  3.9}$}
\\
\hline\hline
Measured Value& \multicolumn{1}{c}{ 2.43}
& \multicolumn{1}{c}{ 4.04}
& \multicolumn{1}{c}{ 6.05}
& \multicolumn{1}{c}{ 7.37}
& \multicolumn{1}{c}{ 8.38}
& \multicolumn{1}{c}{ 9.19}
& \multicolumn{1}{c}{10.07}
& \multicolumn{1}{c}{11.23}
& \multicolumn{1}{c}{12.08}
& \multicolumn{1}{c}{12.77}
& \multicolumn{1}{c}{14.86}
\\
\end{tabular}
\caption{A summary of all the systematic uncertainties and their impact on the $n_\text{track}$ mean for $p_\text{T}^\text{track}>5$ GeV and the more forward jet.  Uncertainties are given in percent. A value of 0.0 is quoted if the uncertainty is below 0.05\%.}
\label{tab:systs_Mean_all_Forward_7}
\end{table} 

